Multiuser Detection by MAP Estimation with Sum-of-Absolute-Values Relaxation

In this article, we consider multiuser detection that copes with multiple access interference caused in star-topology machine-to-machine (M2M) communications. We assume that the transmitted signals are discrete-valued (e.g. binary signals taking values of $\pm 1$), which is taken into account as prior information in detection. We formulate the detection problem as the maximum a posteriori (MAP) estimation, which is relaxed to a convex optimization called the sum-of-absolute-values (SOAV) optimization. The SOAV optimization can be efficiently solved by a proximal splitting algorithm, for which we give the proximity operator in a closed form. Numerical simulations are shown to illustrate the effectiveness of the proposed approach compared with the linear minimum mean-square-error (LMMSE) and the least absolute shrinkage and selection operator (LASSO) methods.

==> fig/FB.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(25.9800,23.3500)(4.5200,-27.3500)%
% CIRCLE 2 0 3 0 Black White  
% 4 1800 600 1800 700 1800 700 1800 700
% 
\special{pn 8}%
\special{ar 1800 600 100 100 0.0000000 6.2831853}%
% VECTOR 2 0 3 0 Black White  
% 2 1900 600 2100 600
% 
\special{pn 8}%
\special{pa 1900 600}%
\special{pa 2100 600}%
\special{fp}%
\special{sh 1}%
\special{pa 2100 600}%
\special{pa 2033 580}%
\special{pa 2047 600}%
\special{pa 2033 620}%
\special{pa 2100 600}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2100 400 2100 800
% 
\special{pn 8}%
\special{pa 2100 400}%
\special{pa 2100 800}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2100 800 2500 600
% 
\special{pn 8}%
\special{pa 2100 800}%
\special{pa 2500 600}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2500 600 2100 400
% 
\special{pn 8}%
\special{pa 2500 600}%
\special{pa 2100 400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2500 600 2700 600
% 
\special{pn 8}%
\special{pa 2500 600}%
\special{pa 2700 600}%
\special{fp}%
% VECTOR 2 0 3 0 Black White  
% 2 1300 600 1700 600
% 
\special{pn 8}%
\special{pa 1300 600}%
\special{pa 1700 600}%
\special{fp}%
\special{sh 1}%
\special{pa 1700 600}%
\special{pa 1633 580}%
\special{pa 1647 600}%
\special{pa 1633 620}%
\special{pa 1700 600}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 2200 500 2200 600 5 0 0 0
% \Large{$\int_{0}^T$}
\put(22.0000,-6.0000){\makebox(0,0){\Large{$\int_{0}^T$}}}%
% LINE 2 0 3 0 Black White  
% 2 1729 529 1871 672
% 
\special{pn 8}%
\special{pa 1729 529}%
\special{pa 1871 672}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 1871 529 1729 671
% 
\special{pn 8}%
\special{pa 1871 529}%
\special{pa 1729 671}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2700 600 2850 550
% 
\special{pn 8}%
\special{pa 2700 600}%
\special{pa 2850 550}%
\special{fp}%
% VECTOR 2 0 3 0 Black White  
% 2 2850 600 3050 600
% 
\special{pn 8}%
\special{pa 2850 600}%
\special{pa 3050 600}%
\special{fp}%
\special{sh 1}%
\special{pa 3050 600}%
\special{pa 2983 580}%
\special{pa 2997 600}%
\special{pa 2983 620}%
\special{pa 3050 600}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 1300 600 1300 2400
% 
\special{pn 8}%
\special{pa 1300 600}%
\special{pa 1300 2400}%
\special{fp}%
% CIRCLE 2 0 3 0 Black White  
% 4 1800 2400 1800 2500 1800 2500 1800 2500
% 
\special{pn 8}%
\special{ar 1800 2400 100 100 0.0000000 6.2831853}%
% VECTOR 2 0 3 0 Black White  
% 2 1900 2400 2100 2400
% 
\special{pn 8}%
\special{pa 1900 2400}%
\special{pa 2100 2400}%
\special{fp}%
\special{sh 1}%
\special{pa 2100 2400}%
\special{pa 2033 2380}%
\special{pa 2047 2400}%
\special{pa 2033 2420}%
\special{pa 2100 2400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2100 2200 2100 2600
% 
\special{pn 8}%
\special{pa 2100 2200}%
\special{pa 2100 2600}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2100 2600 2500 2400
% 
\special{pn 8}%
\special{pa 2100 2600}%
\special{pa 2500 2400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2500 2400 2100 2200
% 
\special{pn 8}%
\special{pa 2500 2400}%
\special{pa 2100 2200}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2500 2400 2700 2400
% 
\special{pn 8}%
\special{pa 2500 2400}%
\special{pa 2700 2400}%
\special{fp}%
% VECTOR 2 0 3 0 Black White  
% 2 1300 2400 1700 2400
% 
\special{pn 8}%
\special{pa 1300 2400}%
\special{pa 1700 2400}%
\special{fp}%
\special{sh 1}%
\special{pa 1700 2400}%
\special{pa 1633 2380}%
\special{pa 1647 2400}%
\special{pa 1633 2420}%
\special{pa 1700 2400}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 2200 2300 2200 2400 5 0 0 0
% \Large{$\int_{0}^T$}
\put(22.0000,-24.0000){\makebox(0,0){\Large{$\int_{0}^T$}}}%
% LINE 2 0 3 0 Black White  
% 2 1729 2329 1871 2472
% 
\special{pn 8}%
\special{pa 1729 2329}%
\special{pa 1871 2472}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 1871 2329 1729 2471
% 
\special{pn 8}%
\special{pa 1871 2329}%
\special{pa 1729 2471}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 2700 2400 2850 2350
% 
\special{pn 8}%
\special{pa 2700 2400}%
\special{pa 2850 2350}%
\special{fp}%
% VECTOR 2 0 3 0 Black White  
% 2 2850 2400 3050 2400
% 
\special{pn 8}%
\special{pa 2850 2400}%
\special{pa 3050 2400}%
\special{fp}%
\special{sh 1}%
\special{pa 3050 2400}%
\special{pa 2983 2380}%
\special{pa 2997 2400}%
\special{pa 2983 2420}%
\special{pa 3050 2400}%
\special{fp}%
% VECTOR 2 0 3 0 Black White  
% 2 1800 900 1800 700
% 
\special{pn 8}%
\special{pa 1800 900}%
\special{pa 1800 700}%
\special{fp}%
\special{sh 1}%
\special{pa 1800 700}%
\special{pa 1780 767}%
\special{pa 1800 753}%
\special{pa 1820 767}%
\special{pa 1800 700}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 1800 950 1800 1000 5 0 0 0
% \Large{$h_1(t)$}
\put(18.0000,-10.0000){\makebox(0,0){\Large{$h_1(t)$}}}%
% VECTOR 2 0 3 0 Black White  
% 2 1797 2700 1797 2500
% 
\special{pn 8}%
\special{pa 1797 2700}%
\special{pa 1797 2500}%
\special{fp}%
\special{sh 1}%
\special{pa 1797 2500}%
\special{pa 1777 2567}%
\special{pa 1797 2553}%
\special{pa 1817 2567}%
\special{pa 1797 2500}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 1797 2750 1797 2800 5 0 0 0
% \Large{$h_M(t)$}
\put(17.9700,-28.0000){\makebox(0,0){\Large{$h_M(t)$}}}%
% VECTOR 2 0 3 0 Black White  
% 2 1302 2000 1702 2000
% 
\special{pn 8}%
\special{pa 1302 2000}%
\special{pa 1702 2000}%
\special{fp}%
\special{sh 1}%
\special{pa 1702 2000}%
\special{pa 1635 1980}%
\special{pa 1649 2000}%
\special{pa 1635 2020}%
\special{pa 1702 2000}%
\special{fp}%
% DOT 2 0 3 0 Black White  
% 4 1802 2000 1902 2000 2002 2000 2002 2000
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 1802 2000 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 1902 2000 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 2002 2000 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 2002 2000 8 8 0 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 902 1500 1302 1500
% 
\special{pn 8}%
\special{pa 902 1500}%
\special{pa 1302 1500}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 802 1350 802 1400 5 0 0 0
% \large{$y(t)$}
\put(8.0200,-14.0000){\makebox(0,0){\large{$y(t)$}}}%
% STR 2 0 3 0 Black White  
% 4 3200 450 3200 500 5 0 0 0
% \large{$y_1$}
\put(32.0000,-5.0000){\makebox(0,0){\large{$y_1$}}}%
% STR 2 0 3 0 Black White  
% 4 3200 2250 3200 2300 5 0 0 0
% \large{$y_M$}
\put(32.0000,-23.0000){\makebox(0,0){\large{$y_M$}}}%
% VECTOR 2 0 3 0 Black White  
% 2 1300 1196 1700 1196
% 
\special{pn 8}%
\special{pa 1300 1196}%
\special{pa 1700 1196}%
\special{fp}%
\special{sh 1}%
\special{pa 1700 1196}%
\special{pa 1633 1176}%
\special{pa 1647 1196}%
\special{pa 1633 1216}%
\special{pa 1700 1196}%
\special{fp}%
% DOT 2 0 3 0 Black White  
% 4 1800 1196 1900 1196 2000 1196 2000 1196
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 1800 1196 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 1900 1196 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 2000 1196 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 2000 1196 8 8 0 6.2831853}%
% DOT 2 0 3 0 Black White  
% 4 1800 1495 1800 1595 1800 1695 1800 1695
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 1800 1495 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 1800 1595 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 1800 1695 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 1800 1695 8 8 0 6.2831853}%
\end{picture}}%


==> fig/m2m.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(38.0000,33.0000)(12.0000,-35.0000)%
% BOX 2 0 3 0 Black White  
% 2 2600 1600 3000 2000
% 
\special{pn 8}%
\special{pa 2600 1600}%
\special{pa 3000 1600}%
\special{pa 3000 2000}%
\special{pa 2600 2000}%
\special{pa 2600 1600}%
\special{pa 3000 1600}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3000 1800 3200 1800
% 
\special{pn 8}%
\special{pa 3000 1800}%
\special{pa 3200 1800}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3200 1800 3200 1400
% 
\special{pn 8}%
\special{pa 3200 1800}%
\special{pa 3200 1400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3100 1400 3300 1400
% 
\special{pn 8}%
\special{pa 3100 1400}%
\special{pa 3300 1400}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3300 1400 3200 1600
% 
\special{pn 8}%
\special{pa 3300 1400}%
\special{pa 3200 1600}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3200 1600 3100 1400
% 
\special{pn 8}%
\special{pa 3200 1600}%
\special{pa 3100 1400}%
\special{fp}%
% CIRCLE 2 0 0 0 Black White  
% 4 2000 1000 2000 1100 2000 1100 2000 1100
% 
\special{sh 1.000}%
\special{ia 2000 1000 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2000 1000 100 100 0.0000000 6.2831853}%
% CIRCLE 2 0 3 0 Black White  
% 4 2800 1800 2800 200 2800 200 2800 200
% 
\special{pn 8}%
\special{ar 2800 1800 1600 1600 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black White  
% 4 1800 2000 1800 1900 1800 1900 1800 1900
% 
\special{sh 1.000}%
\special{ia 1800 2000 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1800 2000 100 100 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black White  
% 4 2400 2900 2400 3000 2400 3000 2400 3000
% 
\special{sh 1.000}%
\special{ia 2400 2900 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 2400 2900 100 100 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black White  
% 4 3600 2800 3600 2700 3600 2700 3600 2700
% 
\special{sh 1.000}%
\special{ia 3600 2800 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3600 2800 100 100 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black White  
% 4 3200 2600 3200 2500 3200 2500 3200 2500
% 
\special{sh 1.000}%
\special{ia 3200 2600 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3200 2600 100 100 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black White  
% 4 3200 600 3200 700 3200 700 3200 700
% 
\special{sh 1.000}%
\special{ia 3200 600 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3200 600 100 100 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black White  
% 4 3800 1200 3800 1300 3800 1300 3800 1300
% 
\special{sh 1.000}%
\special{ia 3800 1200 100 100 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 3800 1200 100 100 0.0000000 6.2831853}%
% VECTOR 2 2 3 0 Black White  
% 2 3200 800 3200 1200
% 
\special{pn 8}%
\special{pa 3200 800}%
\special{pa 3200 1200}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 3200 1200}%
\special{pa 3220 1133}%
\special{pa 3200 1147}%
\special{pa 3180 1133}%
\special{pa 3200 1200}%
\special{fp}%
% VECTOR 2 2 3 0 Black White  
% 2 2200 1100 3000 1300
% 
\special{pn 8}%
\special{pa 2200 1100}%
\special{pa 3000 1300}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 3000 1300}%
\special{pa 2940 1264}%
\special{pa 2948 1287}%
\special{pa 2930 1303}%
\special{pa 3000 1300}%
\special{fp}%
% VECTOR 2 2 3 0 Black White  
% 4 3600 1300 3400 1400 3400 1400 3400 1400
% 
\special{pn 8}%
\special{pa 3600 1300}%
\special{pa 3400 1400}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 3400 1400}%
\special{pa 3469 1388}%
\special{pa 3448 1376}%
\special{pa 3451 1352}%
\special{pa 3400 1400}%
\special{fp}%
\special{pa 3400 1400}%
\special{pa 3400 1400}%
\special{dt 0.045}%
% VECTOR 2 2 3 0 Black White  
% 2 3600 2600 3400 1600
% 
\special{pn 8}%
\special{pa 3600 2600}%
\special{pa 3400 1600}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 3400 1600}%
\special{pa 3393 1669}%
\special{pa 3410 1652}%
\special{pa 3433 1661}%
\special{pa 3400 1600}%
\special{fp}%
% VECTOR 2 2 3 0 Black White  
% 2 3300 2400 3300 1600
% 
\special{pn 8}%
\special{pa 3300 2400}%
\special{pa 3300 1600}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 3300 1600}%
\special{pa 3280 1667}%
\special{pa 3300 1653}%
\special{pa 3320 1667}%
\special{pa 3300 1600}%
\special{fp}%
% VECTOR 2 2 3 0 Black White  
% 2 2500 2700 2900 2300
% 
\special{pn 8}%
\special{pa 2500 2700}%
\special{pa 2900 2300}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 2900 2300}%
\special{pa 2839 2333}%
\special{pa 2862 2338}%
\special{pa 2867 2361}%
\special{pa 2900 2300}%
\special{fp}%
% VECTOR 2 2 3 0 Black White  
% 2 2100 1800 2500 1600
% 
\special{pn 8}%
\special{pa 2100 1800}%
\special{pa 2500 1600}%
\special{dt 0.045}%
\special{sh 1}%
\special{pa 2500 1600}%
\special{pa 2431 1612}%
\special{pa 2452 1624}%
\special{pa 2449 1648}%
\special{pa 2500 1600}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 1830 2150 1830 2250 5 0 0 0
% \Large{M2M device}
\put(18.3000,-22.5000){\makebox(0,0){\Large{M2M device}}}%
% STR 2 0 3 0 Black White  
% 4 2800 2050 2800 2150 5 0 0 0
% \Large{gateway}
\put(28.0000,-21.5000){\makebox(0,0){\Large{gateway}}}%
% BOX 2 0 3 0 Black White  
% 2 3800 3100 5000 3500
% 
\special{pn 8}%
\special{pa 3800 3100}%
\special{pa 5000 3100}%
\special{pa 5000 3500}%
\special{pa 3800 3500}%
\special{pa 3800 3100}%
\special{pa 5000 3100}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 4400 3200 4400 3300 5 0 0 0
% \Large{cloud}
\put(44.0000,-33.0000){\makebox(0,0){\Large{cloud}}}%
% LINE 0 0 3 0 Black White  
% 2 3000 1900 4600 3100
% 
\special{pn 20}%
\special{pa 3000 1900}%
\special{pa 4600 3100}%
\special{fp}%
\end{picture}}%


==> fig/prox.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(46.8000,31.0000)(12.0000,-39.0000)%
% LINE 2 0 3 0 Black White  
% 4 1200 2200 5200 2200 5200 2200 5200 2200
% 
\special{pn 8}%
\special{pa 1200 2200}%
\special{pa 5200 2200}%
\special{fp}%
\special{pa 5200 2200}%
\special{pa 5200 2200}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3200 800 3200 3600
% 
\special{pn 8}%
\special{pa 3200 800}%
\special{pa 3200 3600}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 2800 2200 3600 2200
% 
\special{pn 20}%
\special{pa 2800 2200}%
\special{pa 3600 2200}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 3600 2200 4000 1800
% 
\special{pn 20}%
\special{pa 3600 2200}%
\special{pa 4000 1800}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 4000 1800 4400 1800
% 
\special{pn 20}%
\special{pa 4000 1800}%
\special{pa 4400 1800}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 4400 1800 5000 1200
% 
\special{pn 20}%
\special{pa 4400 1800}%
\special{pa 5000 1200}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 2800 2200 2400 2600
% 
\special{pn 20}%
\special{pa 2800 2200}%
\special{pa 2400 2600}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 2400 2600 2000 2600
% 
\special{pn 20}%
\special{pa 2400 2600}%
\special{pa 2000 2600}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 2000 2600 1600 3000
% 
\special{pn 20}%
\special{pa 2000 2600}%
\special{pa 1600 3000}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 3300 2200 3300 2300 5 0 0 0
% \Large{$O$}
\put(33.0000,-23.0000){\makebox(0,0){\Large{$O$}}}%
% STR 2 0 3 0 Black White  
% 4 5100 1900 5100 2000 5 0 0 0
% \Large{$v$}
\put(51.0000,-20.0000){\makebox(0,0){\Large{$v$}}}%
% STR 2 0 3 0 Black White  
% 4 3400 800 3400 900 5 0 0 0
% \Large{$\xi (v)$}
\put(34.0000,-9.0000){\makebox(0,0){\Large{$\xi (v)$}}}%
% STR 2 0 3 0 Black White  
% 4 3000 1700 3000 1800 5 0 0 0
% \Large{$1$}
\put(30.0000,-18.0000){\makebox(0,0){\Large{$1$}}}%
% STR 2 0 3 0 Black White  
% 4 3400 2500 3400 2600 5 0 0 0
% \Large{$-1$}
\put(34.0000,-26.0000){\makebox(0,0){\Large{$-1$}}}%
% LINE 2 2 3 0 Black White  
% 2 3200 1800 4000 1800
% 
\special{pn 8}%
\special{pa 3200 1800}%
\special{pa 4000 1800}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 3200 2600 2400 2600
% 
\special{pn 8}%
\special{pa 3200 2600}%
\special{pa 2400 2600}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 3600 2200 3600 2300 5 0 0 0
% $Q_3$
\put(36.0000,-23.0000){\makebox(0,0){$Q_3$}}%
% STR 2 0 3 0 Black White  
% 4 4000 2200 4000 2300 5 0 0 0
% $Q_4$
\put(40.0000,-23.0000){\makebox(0,0){$Q_4$}}%
% STR 2 0 3 0 Black White  
% 4 4400 2200 4400 2300 5 0 0 0
% $Q_5$
\put(44.0000,-23.0000){\makebox(0,0){$Q_5$}}%
% STR 2 0 3 0 Black White  
% 4 2800 2000 2800 2100 5 0 0 0
% $Q_2$
\put(28.0000,-21.0000){\makebox(0,0){$Q_2$}}%
% STR 2 0 3 0 Black White  
% 4 2400 2000 2400 2100 5 0 0 0
% $Q_1$
\put(24.0000,-21.0000){\makebox(0,0){$Q_1$}}%
% STR 2 0 3 0 Black White  
% 4 2000 2000 2000 2100 5 0 0 0
% $Q_0$
\put(20.0000,-21.0000){\makebox(0,0){$Q_0$}}%
% LINE 2 2 3 0 Black White  
% 2 2400 2200 2400 2600
% 
\special{pn 8}%
\special{pa 2400 2200}%
\special{pa 2400 2600}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 2000 2600 2000 2200
% 
\special{pn 8}%
\special{pa 2000 2600}%
\special{pa 2000 2200}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 4000 2200 4000 1800
% 
\special{pn 8}%
\special{pa 4000 2200}%
\special{pa 4000 1800}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 4400 1800 4400 2200
% 
\special{pn 8}%
\special{pa 4400 1800}%
\special{pa 4400 2200}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 4000 2500 4000 2600 1 0 0 0
% $Q_0 = -1+\gamma(-q_0-q_1-q_2)$
\put(40.0000,-26.0000){\makebox(0,0)[lt]{$Q_0 = -1+\gamma(-q_0-q_1-q_2)$}}%
% STR 2 0 3 0 Black White  
% 4 4000 2700 4000 2800 1 0 0 0
% $Q_1 = -1+\gamma(q_0-q_1-q_2)$
\put(40.0000,-28.0000){\makebox(0,0)[lt]{$Q_1 = -1+\gamma(q_0-q_1-q_2)$}}%
% STR 2 0 3 0 Black White  
% 4 4000 2900 4000 3000 1 0 0 0
% $Q_2 = \gamma(q_0-q_1-q_2)$
\put(40.0000,-30.0000){\makebox(0,0)[lt]{$Q_2 = \gamma(q_0-q_1-q_2)$}}%
% STR 2 0 3 0 Black White  
% 4 4000 3100 4000 3200 1 0 0 0
% $Q_3 = \gamma(q_0+q_1-q_2)$
\put(40.0000,-32.0000){\makebox(0,0)[lt]{$Q_3 = \gamma(q_0+q_1-q_2)$}}%
% STR 2 0 3 0 Black White  
% 4 4000 3300 4000 3400 1 0 0 0
% $Q_4 = 1+\gamma(q_0+q_1-q_2)$
\put(40.0000,-34.0000){\makebox(0,0)[lt]{$Q_4 = 1+\gamma(q_0+q_1-q_2)$}}%
% STR 2 0 3 0 Black White  
% 4 4000 3500 4000 3600 1 0 0 0
% $Q_5 = 1+\gamma(q_0+q_1+q_2)$
\put(40.0000,-36.0000){\makebox(0,0)[lt]{$Q_5 = 1+\gamma(q_0+q_1+q_2)$}}%
% LINE 2 0 3 0 Black White  
% 2 3880 2500 5880 2500
% 
\special{pn 8}%
\special{pa 3880 2500}%
\special{pa 5880 2500}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 3880 2500 3880 3900
% 
\special{pn 8}%
\special{pa 3880 2500}%
\special{pa 3880 3900}%
\special{fp}%
\end{picture}}%


==> fig/relax.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(45.4500,24.0000)(0.5500,-28.0000)%
% LINE 2 0 3 0 Black White  
% 2 1400 1600 4600 1600
% 
\special{pn 8}%
\special{pa 1400 1600}%
\special{pa 4600 1600}%
\special{fp}%
% DOT 2 0 3 0 Black White  
% 2 3000 2400 3000 2400
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 3000 2400 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 3000 2400 8 8 0 6.2831853}%
% DOT 2 0 3 0 Black White  
% 2 2200 2000 2200 2000
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 2200 2000 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 2200 2000 8 8 0 6.2831853}%
% DOT 2 0 3 0 Black White  
% 2 4000 2200 4000 2200
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 4000 2200 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 4000 2200 8 8 0 6.2831853}%
% DOT 2 0 3 0 Black White  
% 2 3000 1400 3000 1400
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 3000 1400 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 3000 1400 8 8 0 6.2831853}%
% DOT 2 0 3 0 Black White  
% 2 2200 1000 2200 1000
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 2200 1000 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 2200 1000 8 8 0 6.2831853}%
% DOT 2 0 3 0 Black White  
% 2 4000 1200 4000 1200
% 
\special{pn 4}%
\special{sh 1}%
\special{ar 4000 1200 8 8 0 6.2831853}%
\special{sh 1}%
\special{ar 4000 1200 8 8 0 6.2831853}%
% LINE 0 0 3 0 Black White  
% 2 3000 1400 2200 1000
% 
\special{pn 20}%
\special{pa 3000 1400}%
\special{pa 2200 1000}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 4000 1200 4600 1000
% 
\special{pn 20}%
\special{pa 4000 1200}%
\special{pa 4600 1000}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 4600 1600 4600 1700 5 0 0 0
% \large{$x$}
\put(46.0000,-17.0000){\makebox(0,0){\large{$x$}}}%
% STR 2 0 3 0 Black White  
% 4 2300 1700 2300 1800 5 0 0 0
% \large{$r_0$}
\put(23.0000,-18.0000){\makebox(0,0){\large{$r_0$}}}%
% STR 2 0 3 0 Black White  
% 4 3100 1700 3100 1800 5 0 0 0
% \large{$r_1$}
\put(31.0000,-18.0000){\makebox(0,0){\large{$r_1$}}}%
% STR 2 0 3 0 Black White  
% 4 4100 1700 4100 1800 5 0 0 0
% \large{$r_2$}
\put(41.0000,-18.0000){\makebox(0,0){\large{$r_2$}}}%
% LINE 0 0 3 0 Black White  
% 2 3000 1400 4000 1200
% 
\special{pn 20}%
\special{pa 3000 1400}%
\special{pa 4000 1200}%
\special{fp}%
% LINE 0 1 3 0 Black White  
% 2 4000 2200 4600 2400
% 
\special{pn 20}%
\special{pa 4000 2200}%
\special{pa 4600 2400}%
\special{da 0.070}%
% LINE 0 1 3 0 Black White  
% 2 4000 2200 3000 2400
% 
\special{pn 20}%
\special{pa 4000 2200}%
\special{pa 3000 2400}%
\special{da 0.070}%
% LINE 0 1 3 0 Black White  
% 2 3000 2400 2200 2000
% 
\special{pn 20}%
\special{pa 3000 2400}%
\special{pa 2200 2000}%
\special{da 0.070}%
% LINE 3 2 3 0 Black White  
% 2 2200 2000 2200 1000
% 
\special{pn 4}%
\special{pa 2200 2000}%
\special{pa 2200 1000}%
\special{dt 0.045}%
% LINE 3 2 3 0 Black White  
% 2 3000 1400 3000 2400
% 
\special{pn 4}%
\special{pa 3000 1400}%
\special{pa 3000 2400}%
\special{dt 0.045}%
% LINE 3 2 3 0 Black White  
% 2 4000 1200 4000 2200
% 
\special{pn 4}%
\special{pa 4000 1200}%
\special{pa 4000 2200}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 1100 2400 1100 2500 5 0 0 0
% \large{$\log p_0 + \log p_2$}
\put(11.0000,-25.0000){\makebox(0,0){\large{$\log p_0 + \log p_2$}}}%
% STR 2 0 3 0 Black White  
% 4 1100 2200 1100 2300 5 0 0 0
% \large{$\log p_0 + \log p_1$}
\put(11.0000,-23.0000){\makebox(0,0){\large{$\log p_0 + \log p_1$}}}%
% STR 2 0 3 0 Black White  
% 4 1100 2000 1100 2100 5 0 0 0
% \large{$\log p_1 + \log p_2$}
\put(11.0000,-21.0000){\makebox(0,0){\large{$\log p_1 + \log p_2$}}}%
% LINE 3 2 3 0 Black White  
% 2 1600 2400 3000 2400
% 
\special{pn 4}%
\special{pa 1600 2400}%
\special{pa 3000 2400}%
\special{dt 0.045}%
% LINE 3 2 3 0 Black White  
% 2 4000 2200 1600 2200
% 
\special{pn 4}%
\special{pa 4000 2200}%
\special{pa 1600 2200}%
\special{dt 0.045}%
% LINE 3 2 3 0 Black White  
% 2 2200 2000 1600 2000
% 
\special{pn 4}%
\special{pa 2200 2000}%
\special{pa 1600 2000}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 900 1400 900 1500 5 0 0 0
% \large{$\log p_0 + \log p_2 + C$}
\put(9.0000,-15.0000){\makebox(0,0){\large{$\log p_0 + \log p_2 + C$}}}%
% STR 2 0 3 0 Black White  
% 4 900 1200 900 1300 5 0 0 0
% \large{$\log p_0 + \log p_1 + C$}
\put(9.0000,-13.0000){\makebox(0,0){\large{$\log p_0 + \log p_1 + C$}}}%
% STR 2 0 3 0 Black White  
% 4 900 1000 900 1100 5 0 0 0
% \large{$\log p_1 + \log p_2 + C$}
\put(9.0000,-11.0000){\makebox(0,0){\large{$\log p_1 + \log p_2 + C$}}}%
% LINE 3 2 3 0 Black White  
% 2 1600 1000 2200 1000
% 
\special{pn 4}%
\special{pa 1600 1000}%
\special{pa 2200 1000}%
\special{dt 0.045}%
% LINE 3 2 3 0 Black White  
% 2 1600 1200 4000 1200
% 
\special{pn 4}%
\special{pa 1600 1200}%
\special{pa 4000 1200}%
\special{dt 0.045}%
% LINE 3 2 3 0 Black White  
% 2 3000 1400 1600 1400
% 
\special{pn 4}%
\special{pa 3000 1400}%
\special{pa 1600 1400}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 4000 700 4000 800 5 0 0 0
% \large{$\displaystyle{\sum_{l=0}^L q_l\|x-r_l\|_1}$}
\put(40.0000,-8.0000){\makebox(0,0){\large{$\displaystyle{\sum_{l=0}^L q_l\|x-r_l\|_1}$}}}%
% STR 2 0 3 0 Black White  
% 4 4000 2500 4000 2600 5 0 0 0
% \large{$\displaystyle{\sum_{l=0}^L (\log p_l)\|x-r_l\|_1}$}
\put(40.0000,-26.0000){\makebox(0,0){\large{$\displaystyle{\sum_{l=0}^L (\log p_l)\|x-r_l\|_1}$}}}%
% LINE 0 0 3 0 Black White  
% 2 2200 1000 1800 400
% 
\special{pn 20}%
\special{pa 2200 1000}%
\special{pa 1800 400}%
\special{fp}%
% LINE 0 1 3 0 Black White  
% 2 2200 2000 1800 2800
% 
\special{pn 20}%
\special{pa 2200 2000}%
\special{pa 1800 2800}%
\special{da 0.070}%
\end{picture}}%

